A Transformation-based Implementation for CLP with Qualification and Proximity

Uncertainty in logic programming has been widely investigated in the last decades, leading to multiple extensions of the classical LP paradigm. However, few of these are designed as extensions of the well-established and powerful CLP scheme for Constraint Logic Programming. In a previous work we have proposed the SQCLP ({\em proximity-based qualified constraint logic programming}) scheme as a quite expressive extension of CLP with support for qualification values and proximity relations as generalizations of uncertainty values and similarity relations, respectively. In this paper we provide a transformation technique for transforming SQCLP programs and goals into semantically equivalent CLP programs and goals, and a practical Prolog-based implementation of some particularly useful instances of the SQCLP scheme. We also illustrate, by showing some simple---and working---examples, how the prototype can be effectively used as a tool for solving problems where qualification values and proximity relations play a key role. Intended use of SQCLP includes flexible information retrieval applications.

==> J0.tex <==
% ----
% Section 0: Provisional
% ----
\section{Provisional}
\label{sec:provisional}

\subsection{Collection of references to related work}
% Temporal subsection. To be removed later.
% Rubio09 hace referencia al proyecto de tesis de Clemente Rubio.

\begin{enumerate}
%
% LOGIC PROGRAMMING
%
\item
General references on classical LP: \citep{Llo87,Apt90}.
\item
Classical results on LP semantics: \citep{VEK76,AVE82}.
\item
Open Herbrand model semantics (C-semantics) for LP: \citep{Cla79,FLMP93}. 
\item
S-semantics for LP: \citep{FLMP89}.      % NUEVA. Es [33] de LRV07.
\item
Concise presentation of the C- and S-semantics for LP: \citep{AG94}.
\item
Survey on the S-semantics approach for LP: \citep{BGLM94}.      % NUEVA. Es [16] de LRV07.
%
% CONSTRAINT LOGIC PROGRAMMING
%
\item
Seminal paper introducing CLP: \citep{JL87}.     % NUEVA. Es [54] de LRV07.
\item
The CLP scheme of H\"{o}feld and Smolka: \citep{HS88}.     % NUEVA. Aparece en Rie98phd, pg. 140,  con el titulo "Definite relations over constraint languages ..."
\item
The notion of Constraint System aa entailment relation by Saraswat \citep{Sar92} % NUEVA. Se indica debajo:
% Vijay A. Saraswat: The Category of Constraint Systems is Cartesian-Closed LICS 1992: 341-345
\item
Survey on CLP: \citep{JM94}.
\item
Semantics of CLP by Jaffar et al.: \citep{JMM+98}.
\item
Three kinds of semantics for CLP, based on $\pi$-{\em interpretations}, 
and characterizing {\em valid ground goals},  {\em valid answers for goals} and {\em computed answers} for goals, respectively: 
\citep{GL91,GDL95}.
%
% LP and CLP SYSTEMS
%
\item
CLP(R): \citep{JMSY92}.
\item
Prolog III: \citep{Col87}.     % NUEVA. Es [16] de Rubio09.
\item
Chip: \citep{DHS+88}.  % NUEVA. Es [17] de Rubio09.
\item 
Life: \citep{AP93}.   % NUEVA. Es [9] de Rubio09, pero la cita de Rubio09 tiene erratas. Corregir.
\item
Eclipse: \citep{WNS97}.   % NUEVA. Es [89] de Rubio09, pero la cita de Rubio09 tiene erratas. Corregir.
\item
Ciao Prolog: \citep{ciao}.   % NUEVA. Generarla incluyendo una referencia a la web donde esta disponible Ciao.
%
% EFFICIENT IMPLEMENTATION OF LP LANGUAGES: THE WAM
%
\item
Warren's original paper: \citep{War88}.   % NUEVA. Es [88] de Rubio09.
\item
Ait-Kaci's tutorial: \citep{AK91}.   % NUEVA. Es [6] de Rubio09. El nombre del autor tiene una errata, corregir.
\item
Van Roy's paper: \citep{VR93}.   % NUEVA. Es [86] de Rubio09.
%
% LOGIC PROGRAMMING WITH UNCERTAINTY
%
Subramanhian's recollection \citep{Sub07}.
\item
Shapiro's uncertain LP with weighted clauses: \citep{Sha83}.
\item 
van Emden's QLP: \citep{VE86}.
\item 
Subrahmanian's LP with simple annotated clauses: \citep{Sub87,Sub88}.
\item 
Generalized annotated logic programs (GAP) by Kiefer and Subrahmanian \citep{KS92}.
\item
Probabilistic LP and applications to deductive databases: \citep{NS91,NS92,NS93,DS00}.
\item
Probabilistic LP and bayesian networks: \citep{NH95}.
\item
Hybrid probabilistic LP \citep{DS00}.
\item
Probabilistic agent programs \citep{DNS00} and their extension to deal with both time and uncertainty \citep{DKS06}.
\item
Our papers on QLP, SQLP and CFLP: \citep{RR08,CRR08,CRR09TR}.
Our previous work on the $\qlp{\qdom}$ scheme \cite{RR08,RR08TR} revises and generalizes classical work by van Emden \cite{VE86} on uncertainty in logic programming.  Simple annotated logic programs were proposed in \cite{Sub87,Sub88} as an early alternative to \cite{VE86} and later generalized to a much more expressive Theory of Generalized Annotated Logic Programs ($GAP$ for short) \cite{KS92}. As discussed in the concluding section of \cite{RR08}, the semantics of the $\qlp{\qdom}$ semantics has some advantages w.r.t. $GAP$
%
% CONSTRAINT LOGIC PROGRAMMING WITH UNCERTAINTY
%
\item
Riezler's proposal of Quantitative CLP and appliaction to the ambiguity problem in natural language processing: \citep{Rie96,Rie98phd}.
\item
Riezler's proposal of Probabilistic CLP:  \citep{Rie98phd}.
%
% PROBABILISTIC LOGIC PROGRAMMING AND APPLICATIONS TO DATABASES
%
\item
\cite{NS92,NS93}.
%
% FUZZY SETS AND FUZZY LOGIC
%
\item
Seminal paper by Zadeh: \citep{Zad65}.   % NUEVA. Es [91] de Rubio09.
\item
Introductory course on Fuzzy Logic: \citep{NW2000}.  % NUEVA. Es [73] de Rubio09.
\item
Presentations of Fuzzy Logic as a formal multivalued logic: \citep{Pav79,NPM00,Haj98,Haj06}.  % NUEVAS. Son [76,74,30,31] de Rubio09.
%
% POSSIBILISTIC LOGIC AND POSSIBILISTIC LOGIC PROGRAMMING
%
\item
\cite{DP04,DP01}
%
% FUZZY LP BASED ON FUZZY RESOLUTION: SELECTION OF APPROACHES AND APPLICATIONS
%
\item
Fuzzy resolution principle proposed by Lee: \citep{Lee72}.
\item
Prolog-Elf: \citep{IK85}.  % NUEVA. Es [35] de Rubio09.
\item
Evidential reasoning in LP, Fril Prolog : \citep{Bal86,Bal87,BMP95}.    %  BMP95 es NUEVA. Es [11] de Rubio09.
\item
F-Prolog, application to fuzzy data base systems: \citep{LL88,LL89,LL90}.  % NUEVAS. Son [59,60,58] de Rubio09.
\item
Revision of different models of fuzzy LP with fuzzy unification, by P. Vojt\'{a}\v{s} et al.: \citep{VAG01}.
%
% FUZZY LP USING ANNOTATED CLASUSES (ALSO CALLED WEIGHTED CLAUSES)
%
\item
The approaches to uncertain LP  by van Emden \citep{VE86} and Subrahmanian \citep{Sub87,Sub88} can be also placed in this group.
\item
Formalization of fuzzy LP by P. Vojt\'{a}\v{s}, providing a wide variety of connectives 
(conjunctors, disjunctors and aggregation operators for clause bodies): \citep{Voj01}.
\item
Multi-adjoint LP (MALP), providing different lattices of truth values and various adjoint pairs, each consisting of an implication and a conjunction.
Adjoint pairs allow to formalize the semantics of weighted program clauses in MALP. \citep{MOV01a,MOV01b,MOV04}.
\item
The Fuzzy Prolog \citep{VGM02,GMV04} % VGM02 es NUEVA. Es [27] en GMV04.
using Borel sets as fuzzy truth values and aggregation operators to propagate truth values to the head from the body,
thus giving a semantics to program clauses. acts have attached a truth value. Clauses with non-empty body have attached an aggregation operator. 
The formalization of semantics is unsatisfactory. The implementation is by translation to CLP(R) (supported by the Ciao Prolog system \citep{ciao}).
No formal proof of correctness for the implementation is provided.
\item
Comparison between GAP \citep{KS92} and fuzzy LP with weighted clauses: \citep{KLV04}.
%
% FUZZY UNIFICATION USING FUZZY SETS RATHER THAN SIMILARITY RELATIONS
%
\item 
Fuzzy unification using fuzzy sets rather than similarity relations: \citep{AG98,RFS95,Vir91}. % NUEVAS. Son [7,78,83] de Rubio09.
%
% SIMILARITY AND PROXIMITY RELATIONS. NOTION AND CONSTRUCTION.
%
\item
Notion of similarity relation, by Zadeh: \citep{Zah70}.    % NUEVA. Es [9] de SM99, que a su vez es [81] de Rubio09.
\item 
Notion of proximity relation, generalizing similarity relation: \citep{DP80}.  % NUEVA. Es [5] de SM99, que a su vez es [81] de Rubio09.
\item
Proximity relations  in the fuzzy relational database model: \citep{SM99}.    % NUEVA. Es  [81] de Rubio09.
\item
Efficient transitive closure computation: \citep{Nau95}.   % NUEVA. Es [75] de Rubio09.
\item
Method for computing the transitive closure of fuzzy relations: \citep{GCCS99}. % NUEVA. Es [27] de Rubio09.
\item
A procedure for the construction of a similarity relation from similarity equations: \citep{Jul08}.  % NUEVA. Es [48] de Rubio09.
%
% FUZZY LP USING CLASSICAL LP CLAUSES AND SIMILARITY-BASED UNIFICATION
%
\item
\citep{AF99}. Likelog: a logic programming language for flexible data retrieval. F. Arcelli and F. Formato, Proc. SAC'99.
Results: Based on Fuzzy Logic, with $[0,1]$ as the set of fuzzy truth values and $min$ as the t-norm used to interpret $\land$.
Logic language without function symbols, except constants. Similarity relation $\simrel$ defined over predicate symbols and constants.
$\simrel$-based unification as in \cite{FGS00}. In programs, a term may be either a variable or a 'cloud' (set of constants similar to a degree $\lambda$).
Each program has an extended least-Herbrand model (fuzzy set of ground atoms) which is equal to the fuzzy set of ground atoms that can de derived by $\simrel$-based $SLD$ resolution.
\item
\citep{FGS00}. Similarity-based unification. F. Formato and G. Gerla and M. I. Sessa, Fundamenta Informaticae, 2000.
Results: Extension of Martelli and Montanari's unfication algorithm to work mdulo $\simrel$ in a language without function symbols. An extended u.mg. in the sense of this paper can bind a variable to a 'cloud'.
\item
\citep{GS99}. Similarity in Logic Programming. G. Gerla and M.I. Sessa,  Fuzzy Logic and Soft Computing, 1999.
Results: Similarly to \citep{AF99}: Logic Programming for signatures without function symbols (except constants) enhanced with approximate reasoning via a similarity relation $\simrel$, using $[0,1]$ as the set of fuzzy truth values and $min$ as the t-norm used to interpret $\land$;  notion of fuzzy least Herbrand model.
In Sessa's opinion, the heuristic technique to compute the weights for clauses hardly works and does not share the logical feature of a Prolog system, while the approach in this paper allows to avoid both the introduction of weights in the clauses and the use of fuzzy sets as elements of the language.
Novelty w.r.t. \citep{AF99}: two program transformations, named {\em extended} ($H_\lambda(\Prog)$) and {\em abstract} ($\Prog_\lambda$) defined for any fixed $\lambda \in (0,1]$. (Idea: $H_\lambda(\Prog)$ is the set of all clauses $\simrel$-similar to clauses in $\Prog$ to a degree $\geq \lambda$, while $\Prog_\lambda$ is obtained from $\Prog$ by replacing the signature symbols in all clauses by new symbols that stand for equivalence clases modulo $\simrel$-similarity to a degree $\geq \lambda$). The least Herbrand models of both transformed programs are equivalent and can be used to define the fuzzy least Herbrand model of $\Prog$. Moreover, $SLD$ resolution with respect to both translated programs leads to equivalent results and can be used to implement $\simrel$-based computations with the original program.
\item
\citep{Ses01}. Translations and similarity-based logic programming. M. I. Sessa. Soft Computing, 2001.
Results: The approach in \cite{GS99} is extended to languages with function symbols.
\item
Similarity-based resolution rule by Fontana and Formato: \citep{FF02}.   %  NUEVA: Es [24] de Rubio09.
\item
\citep{Ses02}. Approximate reasoning by similarity-based $SLD$ resolution. M. Sessa, TCS, 2002.
Results: The approach in the two previous papers \citep{GS99,Ses01} is presented and extended with a proposal of $SLD$-resolution with $\simrel$-based unification. The approach works for signatures with function symbols. The extended unification algorithm from \cite{FGS00} is generalized to signatures with function symbols and simplified so that substitutions map variables to terms (rather than 'clouds'). MGUs are computed with some unification degree $\lambda \in (0,1]$ modulo $\simrel$.
$\simrel$-based $SLD$ resolution using $\Prog$ is claimed to be sound and complete w.r.t. classical $SLD$ resolution using $H_\lambda(\Prog)$ (Proposition 7.1) and also w.r.t.  classical $SLD$ resolution using $\Prog_\lambda$ (prop. 7.2). Due to these results, $\simrel$-based $SLD$ resolution can be used to implement $\simrel$ based computations while avoiding the transformation of the program $\Prog$. The soundness part (i) of Proposition 7.1 claims that any substitution $\sigma$ computed with approximation degree $\lambda \in (0,1]$ by $\simrel$-based $SLD$ resolution w.r.t. program $\Prog$ can be also computed by using classical $SLD$ resolution w.r.t. $H_\lambda(\Prog)$. This result can fail in the case that $\Prog$ includes some clause with a non-linear head, as shown by a counterexample in \citep{CRR08}. Intuitively, this does not really mean that $\simrel$-based $SLD$ resolution is incorrect, but rather that the $H_\lambda(\Prog)$ transformation provides an incomplete specification of $\Prog$'s fuzzy semantics.
\item 
\citep{LSS04}. Similarity-based {SLD} resolution and its role for web knowledge discovery. V. Loia, S. Senatore and M. I. Sessa, Fuzzy Sets and Systems, 2004.
\item
Other approaches to the implementation of SLP by program tranasformation.
Using MALP: \citep{MOV04}. Using QLP: \citep{CRR08}.
\item 
The SLP language Bausi-Prolog and its SWAM implementation: \citep{JR06a,JR06b,JRG08a,JRG08b,JR08}. % NUEVAS. Son [51,52,46,49,50] en Rubio09.
\item
Functional logic programming with similarity-based unification: \citep{MP06a,MP07}.
%
% APPLICATIONS TO INFORMATION RETRIEVAL
%
\item
Miyamoto's paper on information retrieval based on fuzzy associations: \citep{Miy90}.  %  NUEVA. Es [66] de Rubio09.
\item
Sessa's paper on flexible querying in deductive databases: \citep{Ses00}. % NUEVA. Es [79] de Rubio09.
\end{enumerate} 

\subsection{Real Introduction}
% Temporal subsection. To be removed later.


% Motivation and general aims of this paper.

Nowadays the term {\em Soft Computing} refers to a research area dealing with the management of uncertain and imprecise information. Among other issues, soft computing includes research on uncertainty in logic programming, which has evolved during the last 25 years, dealing with various approaches to semantics, as well as different applications. The aim of this paper is [TO BE COMPLETED]

% Historical Evolution of  Uncertain Logic Programming.

A recent recollection \cite{Sub07} highlights some phases in the evolution of {\em Uncertain Logic Programming} from the viewpoint of a committed researcher.
Early approaches include the quantitative  treatment of uncertainty in the spirit of
fuzzy logic, as in van Emden's classical paper \cite{VE86} and two
subsequent papers by Subrahmanian \cite{Sub87,Sub88}. The main
contribution of \cite{VE86} was a rigorous declarative semantics for
a $LP$ language with program clauses  of the form $A \qgets{d}
\tup{B}$, where the head $A$ is an atom, the body $\tup{B}$ is a
conjunction of atoms, and the so-called {\em attenuation} factor $d
\in (0,1]$ attached to the clause's implication is used to propagate
to the head the certainty factor $d \times b$, where $b$ is the
minimum of the certainty factors $d_i \in (0,1]$ previously computed
for the various atoms occurring in the body. The papers
\cite{Sub87,Sub88} proposed to use a special lattice $\SL$ in place
of the lattice of the real numbers in the interval $[0,1]$ under
their natural ordering. $\SL$ includes two isomorphic copies of
$[0,1]$ whose elements are incomparable under $\SL$'s ordering and
can be used separately to represent degrees of {\em truth} and {\em
falsity}, respectively, thus enabling a simple treatment of
negation. Other main contributions of \cite{Sub87,Sub88} were the
introduction of annotated program clauses and goals (later
generalized to a much more expressive framework in \cite{KS92}), as
well as goal solving procedures more convenient and powerful than
those given  in \cite{VE86}.

\begin{center}
[TO BE CONTINUED]
\end{center}

% The problem faced in this paper. Its importance. Related work.

% Main contributions  of this paper. Their originality and difficulty.


% Possible applications: (a) web searching / information gathering, (b) limiting search spaces, uncertain knowledge representation, (c) expert systems /AI.

% Structure of this paper.


\noindent
TR INTRODUCTION: \\

% Uncertainty in Logic Programming: Historic Evolution.

The investigation of uncertainty in logic programming has proceeded along various lines during the last 25 years. A recent recollection by V. S. Subrahmanian \cite{Sub07} highlights some phases in the evolution of the topic from the viewpoint of a committed researcher.

Research on the field has dealt with various approaches to semantics, as well as different applications. One of the earliest approaches was {\em Quantitative Logic Programming}, $QLP$ for short. This can be traced back to a paper by Shapiro \cite{Sha83}, who proposed to use real numbers in the interval $(0,1]$ as {\em certainty factors}, as well as {\em certainty functions} for propagating certainty factors from the bodies to the heads of program clauses. Subsequently, van Emden \cite{VE86} considered $QLP$ with an  {\em attenuation factor} $f \in (0,1]$ attached to the implication of each program clause and restricted his attention to the certainty function which propagates to a clause head the certainty factor $f \times b$, where $f$ is the clause's attenuation factor and $b$ is the minimum of the certainty factors known for the body atoms. Van Emden's approach was less general than Shapiro's because of the fixed  choice of a particular certainty function, but it allowed to prove more general results on model theoretic and fixpoint semantics, similar to those previously obtained in \cite{VEK76,AVE82} for classical Logic Programming. Moreover, \cite{VE86} gave a procedure for computing the certainty of atoms in the least Herbrand model of a given program, by applying an alpha-beta heuristic to the atoms' and/or search trees. This procedure worked only for ground atoms having a finite search tree.

Following these beginnings, logic programming with uncertainty developed in various directions. Subrahmanian \cite{Sub87} proposed an alternative to \cite{VE86}, using a different lattice of numeric values (aiming at a separate representation of certainty degrees for truth an falsity) as well as clauses whose atoms were annotated with values from this lattice. Neither certainty functions nor attenuation factors were used in this approach, which was extended in \cite{Sub88} to provide goal solving procedures enjoying stronger soundness and completeness results. As a brief summary of some significant later contributions let us mention: generalized {\em annotated logic programs} \cite{KS92}, a quite general framework which will be discussed in more detail in Section \ref{Conclusions}; semantics based on {\em bilattices} of generalized truth values with both a `knowledge' order and a `truth' order \cite{Fit91}; logic programming with probabilistic semantics and applications to deductive databases \cite{NS92,NS93}; quantitative and probabilistic constraint logic programming and applications to natural language processing \cite{Rie98phd}; {\em hybrid probabilistic programs} \cite{DS00}; probabilistic agent programs \cite{DNS00} and their extension to deal with both time and uncertainty \cite{DKS06}; logic programs with similarity based unification and applications to flexible data retrieval
\cite{AF99,Ses02,GMV04,LSS04}; and functional logic programming with similarity based unification \cite{MP06a}.

% Aims of the present technical report.

We are interested in a long-term research project aiming at a generalization of existing work on logic  programming with uncertainty.
The generalization we plan to develop will operate in two directions:
a) extending logic programming languages to  more expressive multi-paradigm declarative languages supporting {\em functions} and {\em constraints};
and b) generalizing uncertain truth values to so-called {\em qualification values}, attached to computed answers and intended to
measure the degree in which such computed answers satisfy various user's expectations.
In this setting, (constraint) logic programming with uncertainty becomes the particular case in which no  functional programming features are used and qualification values are just uncertain truth values.
As a first step, we present in this report a generalization  of the early $QLP$ proposal by van Emden \cite{VE86}, which is still appealing because of its neat semantics. Syntactically, our proposal is very close to van Emden's $QLP$: we use qualified definite Horn clauses $A \qgets{d} \tup{B}$ with an attenuation value $d$ attached to the implication and no annotations attached to the atoms. However, we improve \cite{VE86} in the two ways summarized in the abstract: firstly, we replace numeric certainty values (in particular, those playing the role of attenuation factors in program clauses) by  qualification values belonging to a parametrically given {\em Qualification Domain} $\qdom$ with a lattice structure, which provides abstract operations generalizing the use of $min$ (minimum) and $\times$ (product) in \cite{VE86}. In this way we get a {\em generic scheme} $\qlp{\qdom}$. Secondly, we present stronger semantic results and a sound and strongly complete goal solving  procedure called \emph{Qualified $SLD$ Resolution} over $\qdom$(in symbols, SLD($\qdom$)), which extends SLD resolution using {\em annotated atoms} and {\em qualification constraints} over $\qdom$. The $\qlp{\qdom}$ scheme enjoys nice semantic properties and has interesting instances that can be efficiently implemented using $CLP$ technology: $\qlp{\qdom}$ programs and goals can be easily translated into $\clp{\cdom{\qdom}}$ for any choice of a constraint domain $\cdom{\qdom}$ able to compute with qualification constraints
over $\qdom$.

% Structure of the technical report.

We have developed a prototype implementation of some instances of the $\qlp{\qdom}$ scheme
(including  van Emden's $QLP$) on top of the $CFLP$ system $\toy$.

After this introduction, the rest of the report is structured as follows: Section \ref{Domains} presents the axioms for qualification domains $\qdom$, showing some basic instances and proving that the class of such domains is closed under cartesian product. Section \ref{Language} presents the syntax and declarative semantics of the $\qlp{\qdom}$ scheme. Section \ref{Solving} presents  qualified $SLD$ resolution over $\qdom$ with its soundness and strong completeness properties. Section \ref{Implementation} presents the general implementation technique for $\qlp{\qdom}$
that we have used to implement some instances  of the scheme (including  van Emden's $QLP$) on top of the $CFLP$ system $\toy$. Finally, Section \ref{Conclusions} presents our conclusions and plans for future work. Appendix \ref{Proofs} includes detailed proofs for the main results. Other proofs that have been ommitted or sketched can be found in \cite{Rom07} (in Spanish). \\

\noindent
PROLE'08 INTRODUCTION: \\

% Uncertainty in Logic Programming: Historic Beginnings.
The historical evolution of research on uncertainty in logic programming  has been described in a recent recollection by V. S. Subrahmanian \cite{Sub07} and briefly  summarized  in the introductory section of \cite{RR08}. Early approaches include the quantitative  treatment of uncertainty in the spirit of fuzzy logic, as in van Emden's classical paper \cite{VE86}, and two subsequent papers by Subrahmanian \cite{Sub87,Sub88}. The main contribution of \cite{VE86} was a rigorous declarative semantics for a $LP$ language with program clauses  of the form $A \qgets{d} \tup{B}$, where the head $A$ is an atom, the body $\tup{B}$ is a conjunction of atoms, and the so-called {\em attenuation} factor $d \in (0,1]$ attached to the clause's implication is used to propagate to the head the certainty factor $d \times b$, where $b$ is the minimum of the certainty factors $d_i \in (0,1]$ previously computed for the various atoms occurring in the body. The papers \cite{Sub87,Sub88} proposed to use a special lattice $\SL$ in place of the lattice of the real numbers in the interval $[0,1]$ under their natural ordering. $\SL$ includes two isomorphic copies of $[0,1]$ whose elements are incomparable under $\SL$'s ordering and can be used separately to represent degrees of {\em truth} and {\em falsity}, respectively, thus enabling a simple treatment of negation. Other main contributions of \cite{Sub87,Sub88} were the introduction of annotated program clauses and goals (later generalized to a much more expressive framework in \cite{KS92}) and the introduction of goal solving procedures more convenient and powerful than those given  in \cite{VE86}.

% Results in our previous FLOPS'08 paper and aims of the present paper.
In a recent paper \cite{RR08} we have revised the approach to {\em Quantitative Logic Programming} ($QLP$ for short) in \cite{VE86}, generalizing it to a generic scheme $\qlp{\qdom}$ for so-called {\em Qualified Logic Programming} over a parametrically given domain $\qdom$, which must be a lattice satisfying certain natural axioms. The class of qualification domains includes the lattice $[0,1]$ used in \cite{VE86} as well as other lattices whose elements can be used to qualify logical assertions in other ways. In  this paper we present an extension of $\qlp{\qdom}$ to a more expressive scheme $\bqlp{\qdom}$ which provides two main novelties w.r.t. \cite{RR08}. Firstly, so-called {\em threshold constraints} are used to impose lower bounds to the qualifications computed for the individual atoms in clause bodies, with the aim of preventing inferences from insufficiently qualified premises. Secondly, a simple kind of negation is supported by the use of {\em marked atoms} $A$\#\true\, and $A$\#\false, where \true\, and \false\, stand for the two classical truth values. Marked atoms can be viewed as logical assertions associated to bivalued predicates, and their degree of validity  can be qualified by elements of a parametrically given qualification domain $\qdom$. In particular, if the given $\qdom$ is the lattice $[0,1]$, qualifying marked atoms with numeric degrees $d \in (0,1]$ is similar to annotating atoms with values of the lattice $\SL$, as proposed in \cite{Sub87,Sub88}. Nevertheless, the present approach differs from \cite{Sub87,Sub88} in two major aspects: a) our framework can operate with any parametrically given qualification domain $\qdom$ instead of the fixed lattice $\SL$; and b) we use attenuated clauses with threshold constraints, whose expressivity is quite different from that of  the annotated clauses used in \cite{Sub87,Sub88}. More comparisons to related work can be found in Section \ref{Conclusions} and in the concluding section of \cite{RR08}.

% Structure of the paper.
As it was the case for $\qlp{\qdom}$, the new scheme $\bqlp{\qdom}$ has a rigorous declarative semantics and a sound and strongly complete goal resolution procedure which can be efficiently implemented using constraint logic programming technology. The rest of this paper is structured as follows: Section \ref{Domains} presents the axioms for qualification domains $\qdom$ and its basic properties, including closure under cartesian product. The axioms have been revised w.r.t. \cite{RR08} with the aim of enabling the technical treatment of threshold constraints in subsequent sections. Section \ref{Language} presents the syntax and declarative semantics of the $\bqlp{\qdom}$ scheme. Section \ref{Solving} presents  a goal solving procedure for $\bqlp{\qdom}$  along with its soundness and strong completeness properties. Section \ref{Implementation} sketches a general implementation technique for $\bqlp{\qdom}$ which can be used to implement useful instances  of the scheme on top of any system that supports sufficient $CLP$ technology. Finally, Section \ref{Conclusions} summarizes conclusions and plans for future work. \\

\noindent
PPDP'08 INTRODUCTION: \\

% Early work on uncertainty in logic programming

The historical evolution of the research on uncertainty in {\em
Logic Programming} ($LP$) has been described in a recent
recollection by V. S. Subrahmanian \cite{Sub07}. Early approaches
include the quantitative  treatment of uncertainty in the spirit of
fuzzy logic, as in van Emden's classical paper \cite{VE86} and two
subsequent papers by Subrahmanian \cite{Sub87,Sub88}. The main
contribution of \cite{VE86} was a rigorous declarative semantics for
a $LP$ language with program clauses  of the form $A \qgets{d}
\tup{B}$, where the head $A$ is an atom, the body $\tup{B}$ is a
conjunction of atoms, and the so-called {\em attenuation} factor $d
\in (0,1]$ attached to the clause's implication is used to propagate
to the head the certainty factor $d \times b$, where $b$ is the
minimum of the certainty factors $d_i \in (0,1]$ previously computed
for the various atoms occurring in the body. The papers
\cite{Sub87,Sub88} proposed to use a special lattice $\SL$ in place
of the lattice of the real numbers in the interval $[0,1]$ under
their natural ordering. $\SL$ includes two isomorphic copies of
$[0,1]$ whose elements are incomparable under $\SL$'s ordering and
can be used separately to represent degrees of {\em truth} and {\em
falsity}, respectively, thus enabling a simple treatment of
negation. Other main contributions of \cite{Sub87,Sub88} were the
introduction of annotated program clauses and goals (later
generalized to a much more expressive framework in \cite{KS92}), as
well as goal solving procedures more convenient and powerful than
those given  in \cite{VE86}.

% Recent work on similarity-based logic programming

A more recent line of research is {\em Similarity-based Logic
Programming}  (briefly, $SLP$) as presented in \cite{Ses02} and
previous related works such as \cite{AF99,GS99,FGS00,Ses01}. This
approach also uses the lattice $[0,1]$ to deal with uncertainty in
the spirit of fuzzy logic. In contrast to approaches based on
annotated clauses, programs in $SLP$ are just sets of definite Horn
clauses as in classical $LP$. However, a {\em similarity relation}
$\simrel$ (roughly, the fuzzy analog of an equivalence relation)
between predicate and function symbols is used to enable the
unification terms that would be not unifiable in the classical
sense, measured by some degree $\lambda \in (0,1]$. There are
different proposals for the operational semantics of $SLP$ programs.
One possibility is to apply  classical $SLD$ resolution w.r.t. a
transformation of the original program \cite{GS99,Ses01,Ses02}.
Alternatively, a $\simrel$-based $SLD$-resolution procedure relying
on $\simrel$-unification can be applied w.r.t. to the original
program, as proposed in \cite{Ses02}. Propositions 7.1 and 7.2 in
\cite{Ses02} state a correspondence between the answers computed by
$\simrel$-based $SLD$ resolution w.r.t. a given logic program
$\Prog$ and the answers computed by classical $SLD$ resolution
w.r.t. the two transformed programs $\extended{\lambda}{\Prog}$
(built by adding to $\Prog$ new clauses $\simrel$-similar to those
in $\Prog$ up to the degree $\lambda \in (0,1]$) and
$\abstracted{\Prog}{\lambda}$ (built by replacing all the function
and predicate symbols in $\Prog$ by new symbols that represent
equivalence classes modulo $\simrel$-similarity up to $\lambda$).
The $SiLog$ system  \cite{LSS04} has been developed to implement
$SLP$ and to support applications related to flexible information
retrieval from the web.

% Results of our previous FLOPS'08 paper.

The aim of the present paper is to show that similarity-based
reasoning can be expressed in $\qlp{\qdom}$, a programming scheme
for {\em Qualified} $LP$ over a parametrically given {\em
Qualification Domain} $\qdom$ recently presented in \cite{RR08} as a
generalization and improvement of the classical approach by van Emden
\cite{VE86} to $Quantitative$ $LP$. Qualification domains are
lattices satisfying certain natural axioms. They include the
lattice $[0,1]$ used both in \cite{VE86} and in \cite{Ses02}, as
well as other lattices whose elements can be used to qualify logical
assertions by measuring their closeness to different kinds of users'
expectations. Programs in $\qlp{\qdom}$ use $\qdom$-attenuated
clauses of the form $A \qgets{d} \tup{B}$ where $A$ is an atom,
$\tup{B}$ a finite conjunction of atoms and $d \in \qdom$ is the
{\em attenuation value} attached to the clause's implication, used
to propagate to the head the {\em qualification value} $d \circ b$,
where $b$ is the infimum in $\qdom$ of the qualification values
$d_i \in \qdom$ previously computed for the various atoms occurring
in the body, and  $\circ$ is an {\em attenuation operator} coming
with $\qdom$. As reported in \cite{RR08,RR08TR}, the classical
results in $LP$ concerning the existence of least Herbrand models of
programs and the soundenss and completeness of the  $SLD$ resolution procedure
(see e.g.\cite{VEK76,AVE82,Apt90}) have been extended to the $\qlp{\qdom}$
scheme, and potentially useful instances of the scheme have been
implemented on top of the {\em Constraint Functional Logic
Programming} ($CFLP$) system $\toy$ \cite{toy}.

% Results of the present paper.

The results presented in this paper can be summarized as follows: we
consider generalized similarity relations over a set $S$ as mappings
$\simrel: S \times S \to D$ taking values in the carrier set $D$ of
an arbitrarily  given qualification domain $\qdom$, and we  extend
$\qlp{\qdom}$ to a more expressive scheme $\sqlp{\simrel}{\qdom}$
with two parameters for programming modulo $\simrel$-similarity
with $\qdom$-attenuated Horn clauses. We present a declarative
semantics for $\sqlp{\simrel}{\qdom}$ and a program transformation
mapping each $\sqlp{\simrel}{\qdom}$-program $\Prog$ into a
$\qlp{\qdom}$-program $\trans{\simrel}{\Prog}$ whose least Herbrand
model corresponds to that of $\Prog$. Roughly,
$\trans{\simrel}{\Prog}$ is built adding to $\Prog$ new clauses
obtained from the original clauses in $\Prog$ by computing various
new heads $\simrel$-similar to a linearized version of the original
head, adding also $\simrel$-similarity conditions $X_i \sim X_j$  to
the body and suitable clauses for  the  new predicate $\sim$ to
emulate $\simrel$-based unification. Thanks to the
$\trans{\simrel}{\Prog}$ transformation, the sound and complete
procedure for solving goals in $\qlp{\qdom}$ by $\qdom$-qualified
$SLD$ resolution and its implementation in the $\toy$ system
\cite{RR08} can be used to implement  $\sqlp{\simrel}{\qdom}$
computations, including as a particular case $SLP$ computations in
the sense of \cite{Ses02}.

% Comparison to the multiadjoint approach by Medina et al.

Another recent proposal for reducing the $SLP$ approach in
\cite{Ses02} to a fuzzy $LP$ paradigm can be found in \cite{MOV04},
a  paper which relies on  the multi-adjoint framework for Logic
Programming (MALP for short) previously proposed in
\cite{MOV01a,MOV01b}. MALP is a quite general framework
supporting $LP$ with {\em weighted program rules} over different
multi-adjoint lattices, each of which provides a particular choice
of operators for implication, conjunction  and aggregation of atoms
in rule bodies. In comparison to the $\qlp{\qdom}$ scheme, the
multi-adjoint framework differs in motivation and scope.
Multi-adjoint lattices and qualification domains are  two different
classes of algebraic structures. Concerning declarative and
operational semantics, there are also some significant differences
between $\qlp{\qdom}$ and MALP. In particular, MALP's goal solving
procedure relies on a costly computation of {\em reductant clauses},
a technique borrowed from \cite{KS92} which can be avoided in
$\qlp{\qdom}$, as discussed in the concluding section of
\cite{RR08}.

In spite of these differences, the results in \cite{MOV04} concerning
the emulation of similarity-based  can be compared to those in the
present paper. Theorem 24 in \cite{MOV04} shows that  every
classical logic  program $\Prog$ can be transformed into a MALP
program $\MAProg$ which can be executed using only syntactical
unification and emulates the successful computations of $\Prog$
using the $SLD$ resolution with $\simrel$-based unification
introduced  in \cite{Ses02}. $\MAProg$ works over a particular
multi-adjoint lattice $\GL$ with carrier set $[0,1]$ and implication
and conjunction operators chosen according to the so-called G\"{o}del's
semantics \cite{Voj01}. $\MAProg$ also introduces clauses for a
binary predicate $\sim$ which emulates $\simrel$-based unification,
as in our transformation $\trans{\simrel}{\Prog}$. Nevertheless,
$\trans{\simrel}{\Prog}$   is defined for a more general class of
programs and uses the $\simrel$-similarity predicate $\sim$ only if
the source program $\Prog$ has some clause whose head is non-linear.
More detailed comparisons between the program transformations
$\trans{\simrel}{\Prog}$,  $\extended{\lambda}{\Prog}$,
$\abstracted{\Prog}{\lambda}$ and $\MAProg$ will be given in
Subsection \ref{sec:RA}.

The rest of the paper is structured as follows: In Section
\ref{Domains} we recall the qualification domains $\qdom$  first
introduced in \cite{RR08} and we define similarity relations
$\simrel$ over an arbitrary qualification domain. In Section
\ref{Language} we recall the scheme $\qlp{\qdom}$ and we introduce
its extension $\sqlp{\simrel}{\qdom}$ with its declarative
semantics, given by a logical calculus which characterizes the least
Herbrand model $\M{\Prog}$ of each $\sqlp{\simrel}{\qdom}$-program
$\Prog$. In Section \ref{Reduction} we define the transformation
$\trans{\simrel}{\Prog}$ of any given
$\sqlp{\simrel}{\qdom}$-program $\Prog$ into a $\qlp{\qdom}$-program
$\trans{\simrel}{\Prog}$ such that $\M{\trans{\simrel}{\Prog}} =
\M{\Prog}$, we give some comparisons to previously known program
transformations, and we illustrate the application of
$\trans{\simrel}{\Prog}$ to similarity-based computation by means of
a simple example. Finally, in Section \ref{Conclusions} we summarize
conclusions and comparisons to related work,
and we point to planned lines of future work.

% Comentarios sobre trabajos relacionados, para reutilizar.

\begin{comment}
Nowadays the term {\em Soft Computing} refers to a research area dealing with the management of uncertain and imprecise information. Among other issues, soft computing includes research dealing with {\em uncertainty in logic programming}, which has evolved during the last 25 years. Some recollections can be found in \cite{Sub07}.

Our previous work on the $\qlp{\qdom}$ scheme \cite{RR08,RR08TR} revises and generalizes classical work by van Emden \cite{VE86} on uncertainty in logic programming.  Simple annotated logic programs were proposed in \cite{Sub87,Sub88} as an early alternative to \cite{VE86} and later generalized to a much more expressive Theory of Generalized Annotated Logic Programs ($GAP$ for short) \cite{KS92}. As discussed in the concluding section of \cite{RR08}, the semantics of the $\qlp{\qdom}$ semantics has some advantages w.r.t. $GAP$

We are aware of the following works on similarity-based logic programming:
\begin{itemize}
\item \cite{AF99}. Likelog: a logic programming language for flexible data retrieval. F. Arcelli and F. Formato, Proc. SAC'99.
Results: Based on Fuzzy Logic, with $[0,1]$ as the set of fuzzy truth values and $min$ as the t-norm used to interpret $\land$.
Logic language without function symbols, except constants. Similarity relation $\simrel$ defined over predicate symbols and constants.
$\simrel$-based unification as in \cite{FGS00}. In programs, a term may be either a variable or a 'cloud' (set of constants similar to a degree $\lambda$).
Each program has an extended least-Herbrand model (fuzzy set of ground atoms) which is equal to the fuzzy set of ground atoms that can de derived by $\simrel$-based $SLD$ resolution.
\item \cite{FGS00}. Similarity-based unification. F. Formato and G. Gerla and M. I. Sessa, Fundamenta Informaticae, 2000.
Results: Extension of Martelli and Montanari's unfication algorithm to work mdulo $\simrel$ in a language without function symbols. An extended u.mg. in the sense of this paper can bind a variable to a 'cloud'.
\item \cite{GS99}. Similarity in Logic Programming. G. Gerla and M.I. Sessa,  Fuzzy Logic and Soft Computing, 1999.
Results: Similarly to \cite{AF99}: Logic Programming for signatures without function symbols (except constants) enhanced with approximate reasoning via a similarity relation $\simrel$, using $[0,1]$ as the set of fuzzy truth values and $min$ as the t-norm used to interpret $\land$;  notion of fuzzy least Herbrand model.
In Sessa's opinion, the heuristic technique to compute the weights for clauses hardly works and does not share the logical feature of a Prolog system, while the approach in this paper allows to avoid both the introduction of weights in the clauses and the use of fuzzy sets as elements of the language.
Novelty w.r.t. \cite{GS99}: two program transformations, named {\em extended} ($H_\lambda(\Prog)$) and {\em abstract} ($\Prog_\lambda$) defined for any fixed $\lambda \in (0,1]$. (Idea: $H_\lambda(\Prog)$ is the set of all clauses $\simrel$-similar to clauses in $\Prog$ to a degree $\geq \lambda$, while $\Prog_\lambda$ is obtained from $\Prog$ by replacing the signature symbols in all clauses by new symbols that stand for equivalence clases modulo $\simrel$-similarity to a degree $\geq \lambda$). The least Herbrand models of both transformed programs are equivalent and can be used to define the fuzzy least Herbrand model of $\Prog$. Moreover, $SLD$ resolution with respect to both translated programs leads to equivalent results and can be used to implement $\simrel$-based computations with the original program.
\item \cite{Ses01} Approximate reasoning by similarity-based {SLD} resolution. M. I. Sessa. Soft Computing, 2001.
Results: The approach in \cite{GS99} is extended to languages with function symbols.
\item \cite{Ses02}. Approximate reasoning by similarity-based $SLD$ resolution. M. Sessa, TCS, 2002.
Results: The approach in the two previous papers \cite{GS99,Ses01} is presented and extended with a proposal of $SLD$-resolution with $\simrel$-based unification. The approach works for signatures with function symbols. The extended unification algorithm from \cite{FGS00} is generalized to signatures with function symbols and simplified so that substitutions map variables to terms (rather than 'clouds'). MGUs are computed with some unification degree $\lambda \in (0,1]$ modulo $\simrel$.
$\simrel$-based $SLD$ resolution using $\Prog$ is claimed to be sound and complete w.r.t. classical $SLD$ resolution using $H_\lambda(\Prog)$ (Proposition 7.1) and also w.r.t.  classical $SLD$ resolution using $\Prog_\lambda$ (prop. 7.2). Due to these results, $\simrel$-based $SLD$ resolution can be used to implement $\simrel$ based computations while avoiding the transformation of the program $\Prog$. The soundness part (i) of Proposition 7.1 claims that any substitution $\sigma$ computed with approximation degree $\lambda \in (0,1]$ by $\simrel$-based $SLD$ resolution w.r.t. program $\Prog$ can be also computed by using classical $SLD$ resolution w.r.t. $H_\lambda(\Prog)$. This result can fail in the case that $\Prog$ includes some clause with a non-linear head, as shown by Example \ref{counterexample} below.
Intuitively, this does not really mean that $\simrel$-based $SLD$ resolution is incorrect, but rather that the $H_\lambda(\Prog)$ transformation provides an incomplete specification of $\Prog$'s fuzzy semantics.
\item \cite{LSS04}. Similarity-based {SLD} resolution and its role for web knowledge discovery. V. Loia, S. Senatore and M. I. Sessa, Fuzzy Sets and Systems, 2004.
\item \cite{GMV04}. Fuzzy Prolog: A new Approach using Soft Constraint Propagation. S. Guadarrama, S. Mu{\~{n}}oz and C. Vaucheret, Fuzzy Sets and Systems, 2004.
\item \cite{MOV04}. Similarity-based Unification: a Multi-adjoint Approach. J. Medina, M. Ojeda-Aciego and P. Vojt\'{a}\v{s}, Fuzzy Sets and Systems, 2004.
\item \cite{JMP06}. Operational/Interpretive Unfolding of Multi-adjoint Logic Programs. By R. Juli\'an, G. Moreno and J. Penabad.
\item \cite{MP06a}. Programming with Fuzzy Logic and Mathematical Functions. G. Moreno and V. Pascual, Proc. WILF'05.
\item \cite{MP06b}. Formal Properties of Needed Narrowing with Similarity Relations. G. Moreno and V. Pascual, Proc. PROLE'06.
\end{itemize}
\end{comment}
